SoK: Analysis of Root Causes and Defense Strategies for Attacks on Microarchitectural Optimizations

Microarchitectural optimizations are expected to play a crucial role in ensuring performance scalability in future technology nodes. However, recent attacks have demonstrated that microarchitectural optimizations, which were assumed to be secure, can be exploited. Moreover, new attacks surface at a rapid pace limiting the scope of existing defenses. These developments prompt the need to review microarchitectural optimizations with an emphasis on security, understand the attack landscape and the potential defense strategies. We analyze timing-based side-channel attacks targeting a diverse set of microarchitectural optimizations. We provide a framework for analysing non-transient and transient attacks, which highlights the similarities. We identify the four root causes of timing-based side-channel attacks: determinism, sharing, access violation and information flow, through our systematic analysis. Our key insight is that a subset (or all) of the root causes are exploited by attacks and eliminating any of the exploited root causes, in any attack step, is enough to provide protection. Leveraging our framework, we systematize existing defenses and show that they target these root causes in the different attack steps.

==> section6_related_work.tex <==
%\vspace{-1.5em}
\section{Related Work}
%\vspace{-.5em}
\label{related_work}

%Pandora~\cite{Pandora}

%Survey of Transient Execution Attacks and Their Mitigations
In~\cite{transient_ecex_attacks_22} a survey over transient execution attacks and mitigation's are presented. In contrast, we present a framework for analysing different types of microarchitectural attacks and their defences.  %Survey of Transient Execution Attacks and Their Mitigations  ~\cite{transient_ecex_attacks_22}
 
In~\cite{sok_hw_defences_21} a systematization of hardware defences for speculative execution attacks is presented based on six critical attack steps. In contrast, we present a framework based on the tree root causes for attacks across different optimizations. %SoK: Hardware Defenses Against Speculative Execution Attacks

%A Survey of Microarchitectural Side-channel Vulnerabilities, Attacks and Defences in Cryptography
 In ~\cite{survey_microarch_21} a systematization of microarchitectural side-channel attacks and defences focusing on cryptographic applications is presented. In contrast, we consider all attacks on the optimizations we study.
 
 % ~\cite{sok_spectre_sw_21}
 %In ~\cite{winter_20}
 In~\cite{Szefer2019} 

-----------------------

FROM OLD VERSION OF DEFENSES:
One first strategy is to leverage the defenses available in the optimizations which speculative execution use, as the BP and $SC$. The branch prediction can be targeted in the $setup$ step to stop the adversary from being able to (mis)train the predictor, see Section \ref{def_branch_predictor}. The defense is only applicable for the attacks which uses the specific predictor resource. Another approach is to target the side-channel where information flow allows the secret to be extracted from the transient domain. In many attacks the $SC$ is used since it can offer the highest bandwidth which makes the defenses discussed in Section \ref{def_cache} applicable. %If the SC is used then any of the defenses discussed for SC can be used, see Section \ref{def_cache}. 
The challenge is to target all microarchitectural resources which could be used to create a side channels. Attacks have demonstrated that a large variety of microarchitectural resources can be used, such as execution units, ports, PHT, MSHR etc. However, by defending the resource which enables the high performance side-channels at least the attack bandwidth can be reduced. In addition, can the threat model be limited since for example using a resource which only have temporal contention, restricts the threat model to SMT.

The second category is HW-based disabling. Selective disabling has been proposed by industry to avoid (mis)training using for example Indirect Branch Restricted Speculation (IBRS), Single Thread Indirect Branch Prediction (STIBP) and Indirect Branch Predictor Barrier (IBPB)~\cite{amd_sw,intel_sw}. Likewise, to avoid Spectre v4 the STL mechanism can also be disabled using Speculative Store Bypass Disable (SSBD) microcode updates from Intel and AMD~\cite{ssbd-amd,intel_sw}. These techniques affects the root causes determinism, sharing and information flow in the predictor, in all the steps where it is used. However, the performance cost is potentially high since the predictions are restricted. Another defensive measure is to limit the threat model by disabling SMT which is recommended by industry~\cite{googledisablesmt,openbsddisablesmt,redhatdisablesmt}. This would affect all root causes for the threat model SMT. However, disabling SMT have potentially high performance cost.

The third category is HW-based isolation. One group of proposals aims to introduce fencing with a low performance cost~\cite{CSF_19,vassena2020automatically}. For example Context-Sensitive Fencing (CSF)~\cite{CSF_19} uses customized decoding from instructions to micro-ops to insert fences after a conditional branch instruction and before a subsequent load instruction. The root cause affected by fences is information flow.

Another group of defenses within HW-based isolation targets temporal isolation by not allowing continued execution without authorization~\cite{NDA_19,SpectreGuard_19,Schwarz2020ConTExTAG} which is similar to a selective barrier but in later stage of the attack. For example NDA (Non-speculative Data Access)~\cite{NDA_19} provide different policies for controlling control flow and data propagation. The root causes affected are determinism, sharing and information flow. Another closely related defense strategy also uses temporal isolation where the execution is delayed~\cite{CondSpec_19,InvSpecDef_19,DOLMAS_21}. Here, the defenses delay to avoiding the access violation which leads to leakage or stall the load which would update $MS$ of $SC$. For example in CondSpec~\cite{CondSpec_19} a load that hits in the $SC$ can read the data and complete its execution while a load that experience a cache miss will be stalled and re-issued later. This affects the root cause access violation and/or information flow. Another solution provides temporal isolation by rolling back the changes~\cite{CleanupSpec}. In CleanUpSpec~\cite{CleanupSpec} the speculative execution is allowed to progress and make changes tot the $SC$ but these are removed in case of miss-speculation. This has been shown to be insufficient in certain conditions~\cite{GhostMinion_21}. This defense affects the root causes determinism and information flow, in the $transmit$ and $receive$ step of the attack. 

One group of proposals within HW-based isolation target spatial isolation by introducing a shadow structure to hold the speculative $MS$ until it is deemed safe~\cite{InvisiSpec_18,SafeSpec_19,MounTrap,GhostMinion_21}. For example in MounTrap~\cite{MounTrap} an L0 filter cache is used for speculative data, which is only allowed to propagate to the rest of the cache hierarchy after commit. This allows the speculation and potential access violation to occur but not affect $MS$ of the $SC$, for example. %Here the access violation is allowed to occur but the transient instructions are isolated until non-transient (safe). 
The root cause which is affected is the information flow from the transient execution to the non-transient execution. The performance cost of the defenses discussed within HW-based isolation depends on how restrictive the the rule set is, where protecting at a later attack step generally leads to more flexibility and lower performance cost \cite{sok_hw_defences_21}. The trade-off is that more possible side-channels can be used for the state transitions $MS_I\rightarrow MS_T$ and $MS_T\rightarrow MS_R$, which makes providing full protection more challenging.

%ADD LATER????
%Some techniques are proposed to reduce the overhead of earlier proposed defences~\cite{Oblivious_20,ClearingTheShadows_20,InvarSpec_20}. For example in  ~\cite{Oblivious_20} allows a secret dependent instructions to execute as long as it does not make state changes.

The fourth category is SW-based defenses, where the affected root cause is mostly information flow. One group of defenses~\cite{retpoline,randpoline_2021,amit2019jumpswitches} aims to avoid the speculation triggered by the the branch prediction. Here, the exploitable indirect branch is replaced by a return instruction, and using the $RSB$ the execution is forced into an infinite loop until speculation has been resolved. To lower the performance cost of the technique both a probabilistic variant, randpoline~\cite{randpoline_2021}, and a HW variant~\cite{amit2019jumpswitches} have been proposed. The root cause information flow is affected in the $setup$ step. A recent paper, RETBLEED~\cite{RETBLEED_22}, have shown that the retpoline strategy only provide partial protection, since it can be circumvented using manipulation of return instructions.% and targeting the $BTB$. 

One second strategy within SW-based defenses is to introduce barriers or fences before the transient execution. Industry proposed the use of the serializing $lfence$ instruction before sensitive parts of the code. In order to improve the usability and performance cost, defenses have been proposed which selectively and automatically chose when to use barriers~\cite{CSF_19,shen2018restricting,oleksenko2018you,vassena2020automatically,koruyeh2020speccfi}. For example Shen et al.~\cite{shen2018restricting} split code into small blocks and insert fences between the entry point and a potentially leaking memory access to defend against Spectre attacks. The root causes affected are determinism, sharing and information flow. %Another approach is to protect the access to the secret using for example Speculative Load Hardening (SLH)~\cite{SLH_18}. The idea in SLH is to check and ensure that loads using branchless code is executing on a valid control-flow path and is supported in LLVM and GCC~\cite{llvm_gcc}.

%One third strategy within SW-based defenses is to protect the secret~\cite{ojogbo2020secure,palit2019mitigating,kiriansky2018speculativeBUFFEROVERFLOWS}. For example Palit et al.~\cite{palit2019mitigating} uses a compiler extension to keep annotated sensitive data encrypted in memory. These defenses affect the information flow and access violation in the $interact$ step. In contrast, Sianipar et al. ~\cite{sianipar2018moving} propose a solution which uses a probabilistic approach where sensitive data is continuously moved between a set of positions, to confuse the adversary. This solution targets the determinism in accessing the secret at a specific position in $interact$.
